Spectroscopic followup of three bright halo stars selected from SDSS and GALEX photometry

We aim to reveal the nature of the Sloan Digital Sky Survey (SDSS) stars: SDSSJ100921.40+375233.9, SDSSJ015717.04+135535.9, and SDSSJ171422.43+283657.2, showing apparently high NUV excesses for their g-z colors, as expected for extremely low-metallicity stars. High resolution (R=60 000) spectra of the stars with a wide wavelength coverage were obtained to determine their chemical compositions with the Tull echelle spectrograph on the 2.7 m telescope at the McDonald Observatory. We derived the spectroscopic parameters Teff =5820+-125 K, log g =3.9+-0.2, and vt =1.1+-0.5 km/s for SDSSJ100921.40+375233.9, Teff=6250+-125 K, log g =3.7+-0.2, and vt =4.0+-0.5 km/s for SDSSJ015717.04+135535.9, and Teff=6320+-125 K, log g =4.1+-0.3, and vt =1.5+-0.5 km/s for SDSS J171422.43+283657.2, and elemental abundances were computed for 21 elements for J100921 and J171422 and for 19 elements for J015717 for the first time. We find metallicities of [Fe/H]= -1.30, -0.94, and -0.80 for SDSSJ100921.40+375233.9, J015717.04+135535.9, and J171422.43+283657.2, respectively. On the basis of calculated abundance ratios for J171422.43+283657.2 and J015717.04+135535.9, we also report that these two program stars have the expected composition of main-sequence halo turnoff stars, but with low-alpha abundances, i.e., the [alpha/Fe] ratio is ~0.0 for J171422.43+283657.2 and ~0.1 for J015717.04+135535.9. The latter one shows typical halo or thick-disk alpha-element abundances, but has a substantial rotational line broadening and vsini=40 +- 0.5 km/s.

==> Sahin_research_high.tex <==
- We performed the first detailed abundance analysis on SDSS J100921.40+375233.9 and
J171422.43+283657.2 for 21 elements and on J015717.04+135535.9 for 19 elements.

- We provide a tool to distinguish extremely metal-poor candidate stars using SDSS and Galex photometry of the stars and Kurucz model atmospheres (Fig.1 in the paper).

- Two of the stars under scrutiny (SDSS J100921.40+375233.9 and J171422.43+283657.2)
appear to lie close to ultra-low metallicity ([Fe/H]=−3.5) population track
(Fig 1 in the paper), with the caveat that the SDSS photometry for them is saturated.

- We report that none of these SDSS stars present ultra-low metallicities. Two
of the stars, J171422.43+283657.2 and J015717.04+135535.9 are found to be two low-α halo stars. 

-An interesting anomaly is noted for J015717.04+135535.9 which exhibits a high
rotational velocity (e.g. 40 km s−1 ), unusual for a halo turnoff star. The star,
J100921 is roughly consistent with thick-disk membership.



